Singular limit of a nonlinear fourth order inhomogeneous equation

In this paper we use the method of matched asymptotic expansions in order to obtain a geometric motion as the singular limit of a nonlinear fourth order inhomogeneous equation.

==> References.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ARTICLES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@article{mimura,
  AUTHOR = {Mimura, M. and Tsujikawa, T.},
  TITLE = {Aggregating pattern dynamicsin a chemotaxis modelincluding growth},
  JOURNAL = {Physica},
  VOLUME = {A 230},
  YEAR = {1996},
  PAGES = {499--543},
 }


@article {modica_mortola,
    AUTHOR = {Modica, L. and Mortola, S.},
     TITLE = {Un esempio di {$\Gamma ^{-}$}-convergenza},
   JOURNAL = {Boll. Un. Mat. Ital. B (5)},
    VOLUME = {14},
      YEAR = {1977},
    NUMBER = {1},
     PAGES = {285--299},
   MRCLASS = {49A50},
  MRNUMBER = {0445362 (56 \#3704)},
MRREVIEWER = {Francesco Barbieri}, }



@article {modica_mortola2,
    AUTHOR = {Modica, L.},
     TITLE = {The gradient theory of phase transitions and the minimal
              interface criterion},
   JOURNAL = {Arch. Rational Mech. Anal.},
  FJOURNAL = {Archive for Rational Mechanics and Analysis},
    VOLUME = {98},
      YEAR = {1987},
    NUMBER = {2},
     PAGES = {123--142},
      ISSN = {0003-9527},
     CODEN = {AVRMAW},
   MRCLASS = {76T05 (80A15)},
  MRNUMBER = {866718 (88f:76038)},
MRREVIEWER = {L. Hsiao},
       DOI = {10.1007/BF00251230},
       URL = {http://dx.doi.org/10.1007/BF00251230},
}



@article {ajm,
    AUTHOR = {Alessio, F. and Jeanjean, L. and Montecchiari,
              P.},
     TITLE = {Stationary layered solutions in {$\bold R^2$} for a class
              of non autonomous {A}llen-{C}ahn equations},
   JOURNAL = {Calc. Var. Partial Differential Equations},
  FJOURNAL = {Calculus of Variations and Partial Differential Equations},
    VOLUME = {11},
      YEAR = {2000},
    NUMBER = {2},
     PAGES = {177--202},
      ISSN = {0944-2669},
   MRCLASS = {35J60 (34C37 35J20 37J45)},
  MRNUMBER = {1782992 (2001i:35077)},
MRREVIEWER = {Maria Letizia Bertotti},
       DOI = {10.1007/s005260000036},
       URL = {http://dx.doi.org/10.1007/s005260000036},
}


@article {chen,
    AUTHOR = {Chen, X.},
     TITLE = {Generation and propagation of interfaces for
              reaction-diffusion equations},
   JOURNAL = {J. Differential Equations},
  FJOURNAL = {Journal of Differential Equations},
    VOLUME = {96},
      YEAR = {1992},
    NUMBER = {1},
     PAGES = {116--141},
      ISSN = {0022-0396},
     CODEN = {JDEQAK},
   MRCLASS = {35K57 (35B40 35K15)},
  MRNUMBER = {1153311 (92m:35129)},
MRREVIEWER = {Alan V. Lair},
       DOI = {10.1016/0022-0396(92)90146-E},
      URL = {http://dx.doi.org/10.1016/0022-0396(92)90146-E},
}

@article {cen,
    AUTHOR = {Cahn, J. W. and Elliott, C. M. and Novick-Cohen, A.},
     TITLE = {The {C}ahn-{H}illiard equation with a concentration dependent
              mobility: motion by minus the {L}aplacian of the mean
              curvature},
   JOURNAL = {European J. Appl. Math.},
  FJOURNAL = {European Journal of Applied Mathematics},
    VOLUME = {7},
      YEAR = {1996},
    NUMBER = {3},
     PAGES = {287--301},
      ISSN = {0956-7925},
   MRCLASS = {80A22 (35Q99)},
  MRNUMBER = {1401172 (97g:80010)},
MRREVIEWER = {J. R. Ockendon},
       DOI = {10.1017/S0956792500002369},
       URL = {http://dx.doi.org/10.1017/S0956792500002369},
}



@book {gilbarg_trudinger,
    AUTHOR = {Gilbarg, D. and Trudinger, N. S.},
     TITLE = {Elliptic partial differential equations of second order},
      NOTE = {Grundlehren der Mathematischen Wissenschaften, Vol. 224},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {Berlin},
      YEAR = {1977},
     PAGES = {x+401},
      ISBN = {3-540-08007-4},
   MRCLASS = {35-02 (35J25 35J65)},
  MRNUMBER = {0473443 (57 \#13109)},
MRREVIEWER = {O. John},
}
		

@incollection {DeGiorgi,
    AUTHOR = {De Giorgi, E.},
     TITLE = {Some remarks on {$\Gamma$}-convergence and least squares
              method},
 BOOKTITLE = {Composite media and homogenization theory ({T}rieste, 1990)},
    SERIES = {Progr. Nonlinear Differential Equations Appl.},
    VOLUME = {5},
     PAGES = {135--142},
 PUBLISHER = {Birkh\"auser Boston},
   ADDRESS = {Boston, MA},
      YEAR = {1991},
   MRCLASS = {49J45},
  MRNUMBER = {1145748 (92k:49022)},
MRREVIEWER = {Constantin Z{\u{a}}linescu},
}


@article {LM,
    AUTHOR = {Loreti, P. and March, R.},
     TITLE = {Propagation of fronts in a nonlinear fourth order equation},
   JOURNAL = {European J. Appl. Math.},
  FJOURNAL = {European Journal of Applied Mathematics},
    VOLUME = {11},
      YEAR = {2000},
    NUMBER = {2},
     PAGES = {203--213},
      ISSN = {0956-7925},
   MRCLASS = {58E12 (80A22)},
  MRNUMBER = {1757511 (2001g:58027)},
MRREVIEWER = {Silvano Delladio},
       DOI = {10.1017/S0956792599004131},
      URL = {http://dx.doi.org/10.1017/S0956792599004131},
}


@article {BL,
    AUTHOR = {Lou, B.},
     TITLE = {Singular limit of a {$p$}-{L}aplacian reaction-diffusion
              equation with a spatially inhomogeneous reaction term},
   JOURNAL = {J. Statist. Phys.},
  FJOURNAL = {Journal of Statistical Physics},
    VOLUME = {110},
      YEAR = {2003},
    NUMBER = {1-2},
     PAGES = {377--383},
      ISSN = {0022-4715},
     CODEN = {JSTPSB},
   MRCLASS = {35K57 (35B25 35C20)},
  MRNUMBER = {1966333 (2004b:35189)},
       DOI = {10.1023/A:1021083015108},
       URL = {http://dx.doi.org/10.1023/A:1021083015108},
}


@article {MD,
   AUTHOR = {March, R. and Dozio, M.},
   TITLE = {A variational method for the recovery of smooth
   boundaries},
   JOURNAL = {Image and Vision Computing},
   VOLUME = {15},
   PAGES = {705--712},
   YEAR ={1997},
}



@article {nmhs,
    AUTHOR = {Nakamura, K.-I. and Matano, H. and Hilhorst, D. and
              Sch{\"a}tzle, R.},
     TITLE = {Singular limit of a reaction-diffusion equation with a
              spatially inhomogeneous reaction term},
   JOURNAL = {J. Statist. Phys.},
  FJOURNAL = {Journal of Statistical Physics},
    VOLUME = {95},
      YEAR = {1999},
    NUMBER = {5-6},
     PAGES = {1165--1185},
      ISSN = {0022-4715},
     CODEN = {JSTPSB},
   MRCLASS = {35K57 (92C15)},
  MRNUMBER = {1712446 (2000e:35102)},
       DOI = {10.1023/A:1004518904533},
       URL = {http://dx.doi.org/10.1023/A:1004518904533},
}


@article {pego,
    AUTHOR = {Pego, R. L.},
     TITLE = {Front migration in the nonlinear {C}ahn-{H}illiard equation},
   JOURNAL = {Proc. Roy. Soc. London Ser. A},
  FJOURNAL = {Proceedings of the Royal Society. London. Series A.
              Mathematical, Physical and Engineering Sciences},
    VOLUME = {422},
      YEAR = {1989},
    NUMBER = {1863},
     PAGES = {261--278},
      ISSN = {0962-8444},
     CODEN = {PRLAAZ},
   MRCLASS = {80A20 (35Q20)},
  MRNUMBER = {997638 (90j:80010)},
}




